HP-GNN: Generating High Throughput GNN Training Implementation on CPU-FPGA Heterogeneous Platform

Graph Neural Networks (GNNs) have shown great success in many applications such as recommendation systems, molecular property prediction, traffic prediction, etc. Recently, CPU-FPGA heterogeneous platforms have been used to accelerate many applications by exploiting customizable data path and abundant user-controllable on-chip memory resources of FPGAs. Yet, accelerating and deploying GNN training on such platforms requires not only expertise in hardware design but also substantial development efforts. We propose HP-GNN, a novel framework that generates high throughput GNN training implementations on a given CPU-FPGA platform that can benefit both application developers and machine learning researchers. HP-GNN takes GNN training algorithms, GNN models as the inputs, and automatically performs hardware mapping onto the target CPU-FPGA platform. HP-GNN consists of: (1) data layout and internal representation that reduce the memory traffic and random memory accesses; (2) optimized hardware templates that support various GNN models; (3) a design space exploration engine for automatic hardware mapping; (4) high-level application programming interfaces (APIs) that allows users to specify GNN training with only a handful of lines of code. To evaluate HP-GNN, we experiment with two well-known sampling-based GNN training algorithms and two GNN models. For each training algorithm and model, HP-GNN generates implementation on a state-of-the-art CPU-FPGA platform. Compared with CPU-only and CPU-GPU platforms, experimental results show that the generated implementations achieve $55.67\times$ and $2.17\times$ speedup on the average, respectively. Compared with the state-of-the-art GNN training implementations, HP-GNN achieves up to $4.45\times$ speedup.

==> 4_algo.tex <==
\subsection{Memory Traffic Reduction}
Graphs are usually sparse, and stored in sparse matrix formats such as compressed sparse row/column (CSR/CSC) or coordinate list (COO). In order to reduce the overhead of irregular memory access, our framework choose the COO format as data sorted by source vertices as data layout. During feature aggregation, edges will be streamed in to the aggregation kernel. The aggregation kernel will read the feature vectors of the source vertices from external memory, and send it to the destination vertices for aggregation. Figure \ref{fig:reuse} shows an example of representing a graph in COO format, sorted by source vertices. In this example, feature vector of ${V}_1$ will be send to ${V}_2$, ${V}_4$ and ${V}_5$ for aggregation. Thus, the feature vector of ${V}_1$ can be stored on-chip, and be reused for edge 2 and 3. Similarly, when processing edge 4 and 5, feature vector of ${V}_2$ will be stored on chip and reused. This data layout can avoid loading same feature vectors repeatedly, and thus reduce memory traffic.

\begin{figure}[h]
    \centering
    \includegraphics[width=8.5cm]{pic/reuse.pdf}
    \caption{An example of graph stored in COO format}
     \label{fig:reuse}
\end{figure} 

\subsection{Intermediate Result Buffering}\label{buff}
 When performing aggregation, the feature vectors of the destination vertices will be read, and aggregate with the source feature vectors, and then the intermediate results will be stored back to memory. Since we sort our edges by source instead of destination, reading and storing the intermediate results to the destination vertices will incur irregular memory access with considerable overhead. To mitigate the overhead of memory access, we buffer the feature vectors of destination vertices on-chip. Thus, the irregular access of reading and storing the intermediate results will only be performed on-chip instead of external memory. When the aggregation is finished, the final results will be stored back to external memory sequentially. The size of mini-batch in GNN training ranges from tens to thousands, and the feature dimensions are usually within thousands. Thus, it is feasible to buffer the feature vectors of the destination vertices using FPGA on-chip memory.
 
 \begin{figure}[h]
    \centering
    \includegraphics[width=8.5cm]{pic/SPMM.pdf}
    \caption{Architecture of aggregation kernel}
     \label{fig:SPMM}
\end{figure} 
